Motion Planning for Collision-resilient Mobile Robots in Obstacle-cluttered Unknown Environments with Risk Reward Trade-offs

Collision avoidance in unknown obstacle-cluttered environments may not always be feasible. This paper focuses on an emerging paradigm shift in which potential collisions with the environment can be harnessed instead of being avoided altogether. To this end, we introduce a new sampling-based online planning algorithm that can explicitly handle the risk of colliding with the environment and can switch between collision avoidance and collision exploitation. Central to the planner's capabilities is a novel joint optimization function that evaluates the effect of possible collisions using a reflection model. This way, the planner can make deliberate decisions to collide with the environment if such collision is expected to help the robot make progress toward its goal. To make the algorithm online, we present a state expansion pruning technique that significantly reduces the search space while ensuring completeness. The proposed algorithm is evaluated experimentally with a built-in-house holonomic wheeled robot that can withstand collisions. We perform an extensive parametric study to investigate trade-offs between (user-tuned) levels of risk, deliberate collision decision making, and trajectory statistics such as time to reach the goal and path length.

==> prop1.tex <==
%\begin{proposition}\label{lma2}
%Under the conditions i) of the original optimal steering problem~\cite{chen2016optimal1}, ii) $b_{1_{x},wall}=b_{1_{x},free}$ and $b_{1_{y},wall} \leqslant b_{1_{y},free}$ %for the diffusion coefficients,  and iii) $\sigma_{x,free}(0)=\sigma_{x,wall}(0)$ and $\sigma_{y,free}(0)=\sigma_{y,wall}(0)$, the control energy when interacting with obstacles to navigate through an aperture is less than the control energy to optimally steer the robotic agent directly to target as if there were no obstacles. %of the robot goes from the initial distribution to the final distribution with a finite interval. If the robot interacts with the environmental boundary by performing door entering behavior, the control energy of that robot is less than and equal to the optimal control energy without boundary. 
%\end{proposition} 
%\begin{proof}
Let $k_{x}(t)$ and $k_y(t)$ be as in the linear optimal steering in both free motion and wall-following. The initial distribution and end time stay the same too. When colliding with the wall, the control energy in the $x$ direction is
%
\begin{equation}\label{eq:cost}
\begin{aligned} 
J_{x,wall}=&\int\limits_{0}^{T_{i}}k^{2}_{x}(t)\sigma_{x,wall}(t)dt+\int\limits_{T_{i}}^{T_{d}}k^{2}_{x}(t)\sigma_{x,wall}(t)dt \\
& +\int\limits_{T_{d}}^{T}k^{2}_{x}(t)\sigma_{x,wall}(t)dt \enspace,
\end{aligned} 
\end{equation}
%
where $T_{i}$ and $T_{d}$ denote the time of impact and disengaging from the wall, respectively. 

We can split the control energy required to perform the same task as if there were no obstacles in three parts, according to switching times $T_{i}$ and $T_{d}$.  That is, $J_{x,free} = J_{1}(0\le t \le T_i) + J_{2}(T_i\le t \le T_d) + J_{3}(T_d\le t \le T)$. According to noise kinematics~\eqref{eq11} and due to the condition $\sigma_{x,free}(0)=\sigma_{x,wall}(0)$, then $\sigma_{x,wall}(t)=\sigma_{x,free}(t)$ $t\in [0, T_{i}]$. Hence $J_{1} = \int\limits_{0}^{T_{i}}k^{2}_{x}(t)\sigma_{x,wall}(t)dt$.  Following the same rationale, and assuming that the processes are stationary~\cite{chen2016optimal1} so that we can time swift $J_{3}$ from $t=T_d$ to $t=0$, we get that $J_{3} = \int\limits_{T_{d}}^{T}k^{2}_{x}(t)\sigma_{x,wall}(t)dt$. 
%The Lyapunov differential equation is the same as \eqref{eq8} for the free motion mode. 
%
In wall-following mode the Lyapunov differential equation in $x$ direction is chosen to be 
%
\begin{equation}\label{eq14} %\tag{12a}
\dot{\sigma}_{x,wall}(t)=2b_{x}h_{x}(t)+b_{1_{x},wall}^{2}-Q(t)\enspace.
\end{equation}

$Q(t)$ is added to account for the wall-following effect on $\sigma_{x}(t)$. We consider $Q(t)\geqslant 0$ since the wall-following motion decreases the rate of diffusion over the $x$ direction~\cite{stager2016stochastic}. Therefore, we get $\sigma_{x,wall}(t) \leqslant \sigma_{x, free}(t)$. Then 
%
%\begin{equation}\label{eq12}
\begin{align*}
%J_{2_{x,ape}}& =
\int\limits_{T_{i}}^{T_{d}}k^{2}_{x}(t)\sigma_{x,wall}(t)dt&=\lim \limits_{n\to \infty}\sum \limits_{i=1}^{n} k _{x}^{2}(\xi_{i})\sigma_{x,wall}(\xi_{i})\Delta t \\
& \leqslant  \lim \limits_{n\to \infty}\sum \limits_{i=1}^{n} k _{x}^{2}(\xi_{i})\sigma_{x, free}(\xi_{i})\Delta t\\
&=\int\limits_{T_{i}}^{T_{d}}k^{2}_{x}(t)\sigma_{x, free}(t)dt 
= J_2
\end{align*}
%\end{equation}
%
with $\xi_{i} \in [t_{i}, t_{i+1})$. 
%
Thus, $J_{x,wall} \le J_{x,free}$. 

The same steps apply to the control energy along the $y$ direction. For wall-following when $t\in(T_{i},T_{d}]$, $b_{1_{y}, wall}^{2}\leqslant b_{1_{y},free}^{2}$ and based on the noise kinematics
%
% k^{2}_{x}(\xi)\int\limits_{0}^{T}\sigma_{x, wall}(t) \leqslant k^{2}_{x}(\xi)\int\limits_{0}^{T}\sigma_{x, free}(t)
%
\begin{equation}\label{eq15} %\tag{12b}
\dot{\sigma}_{y,wall}(t)=2b_{y}h_{y}(t)+b_{1_{y},wall}^{2}\enspace,
\end{equation}
%
we get $\sigma_{y,wall}(t) \leqslant \sigma_{y, free}(t)$ leading to 
%
%During the wall-following section $(T_{i},T_{d}]$ $b_{1_{y}, wall}^{2}\leqslant b_{1_{y},free}^{2}$, we get  $\sigma_{y, ape}^{col}(t) \leqslant \sigma_{y, free}(t)$. 
%
%that leads to $J_{y, wall}=\int\limits_{0}^{T}k^{2}_{y}(t)\sigma_{y, wall}(t)=k^{2}_{y}(\xi)\int\limits_{0}^{T}\sigma_{y, wall}(t) \leqslant k^{2}_{y}(\xi)\int\limits_{0}^{T}\sigma_{y, free}(t)$. 
$J_{y, wall} \leqslant J_{y, free}$. 
%
Since motions in the $x$ and $y$ directions are assumed independent from each other, $J_{wall}=J_{x,wall}+J_{y,wall} \le J_{x,free}+J_{y,free}=J_{free}$. %, which concludes the proof.
%\kkb{Combining the motion in both directions we deduce that $J_{2\ x,wall}+J_{2\ y, ape}^{col} \leqslant J_{2\ x, free}+J_{2\ y, free}$.  
%
%Similarly, since $\sigma_{x,ape}^{col}(T_{d}) \leqslant \sigma_{x,free}(T_{d})$ and  $\sigma_{y,ape}^{col}(T_{d}) \leqslant \sigma_{y,free}(T_{d})$, from \eqref{eq12}, the we can get the inequality holds in the disengaging period $(T_{d},T]$.  Hence we get $J_{3\ x, ape}^{col}+J_{3\ y, ape}^{col} \leqslant J_{3\ x, free}+J_{3\ y, free}$ . 
%We can prove that$J_{ape}^{col} \leqslant J_{free}$.}
%\end{proof}

As an immediate consequence, and by the triangle inequality on the system's stochastic process, we get $J_{wall} \le J_{free} \le J_{ncol}$, where $J_{ncol}$ denotes the control energy to steer through the aperture without collision.

%\begin{corollary}\label{col1}
%Piece-wise optimal steering through the aperture within the same time interval requires more energy than interacting with obstacles to navigate through the aperture.
%\end{corollary}
%\begin{proof}
%Let $J_{ncol}$ %=J'_1(0 \le t \le T_{ape}) + J'_2(T_{ape} \le t \le T)$ 
%denote the control energy to steer through the aperture without collision. %, with $T_{ape}$ being the time of passing through the aperture.
%By the triangle inequality on the system's stochastic process, and due to Proposition~\ref{lma2}, we get $J_{wall} \le J_{free} \le J_{ncol}$. % yields $||J_{free}|| \le ||J'_1|| + ||J'_2|| = ||J_{ncol}||$.  proposition~\ref{lma2}, it then follows that
%\kkb{It follows directly from Proposition 1, we get $J_{ape}^{col} \leqslant J_{free}$. Since the feasible set of piece-wise optimal steering  is the subset of optimal steering problem. Then it is easy to prove $J_{ape}^{col} \leqslant J_{free} \leqslant J_{ape}^{ncol}$.}
%\end{proof}
